The crossing multiplier for solvable lattice models

We study the large class of solvable lattice models, based on the data of conformal field theory. These models are constructed from any conformal field theory. We consider the lattice models based on affine algebras described by Jimbo et al., for the algebras $ABCD$ and by Kuniba et al. for $G_2$. We find a general formula for the crossing multipliers of these models. It is shown that these crossing multipliers are also given by the principally specialized characters of the model in question. Therefore we conjecture that the crossing multipliers in this large class of solvable interaction round the face lattice models are given by the characters of the conformal field theory on which they are based. We use this result to study the local state probabilities of these models and show that they are given by the branching rule, in regime III.

==> phyzzx.fonts.tex <==
%
% PHYZZX fonts are kept in this separate file
% in order to facilitate font substitution.
%
% This file should be called PHYZZX.FONTS on sites using CM fonts
% and PHYZZX.CMFONTS on other sites.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\font\teniu=cmu10
\font\seventeenrm =cmr12 scaled\magstep2
\font\fourteenrm  =cmr12 scaled\magstep1
\font\twelverm    =cmr10 scaled\magstep1
\font\tenrm       =cmr8  scaled\magstep1
\font\ninerm      =cmr7  scaled\magstep1
\font\sevenrm     =cmr6  scaled\magstep1
\font\sixrm       =cmr5  scaled\magstep1
\let\fiverm=\sixrm        % no cmr4
%
\font\seventeenbf =cmbx12 scaled\magstep2
\font\fourteenbf  =cmbx12 scaled\magstep1
\font\twelvebf    =cmbx10 scaled\magstep1
\font\tenbf       =cmbx8  scaled\magstep1
\font\ninebf      =cmbx7  scaled\magstep1
\font\sevenbf     =cmbx6  scaled\magstep1
\font\sixbf       =cmbx5  scaled\magstep1
\let\fivebf=\sixbf        % no cmbx4
%
\font\seventeeni  =cmmi12 scaled\magstep2    \skewchar\seventeeni='177
\font\fourteeni   =cmmi12 scaled\magstep1     \skewchar\fourteeni='177
\font\twelvei     =cmmi10 scaled\magstep1       \skewchar\twelvei='177
\font\teni        =cmmi8  scaled\magstep1          \skewchar\teni='177
\font\ninei       =cmmi7  scaled\magstep1         \skewchar\ninei='177
\font\seveni      =cmmi6  scaled\magstep1        \skewchar\seveni='177
\font\sixi        =cmmi5  scaled\magstep1          \skewchar\sixi='177
\let\fivei=\sixi          % no cmmi4
%
\font\seventeensy =cmsy10 scaled\magstep3    \skewchar\seventeensy='60
\font\fourteensy  =cmsy10 scaled\magstep2     \skewchar\fourteensy='60
\font\twelvesy    =cmsy10 scaled\magstep1       \skewchar\twelvesy='60
\font\tensy       =cmsy8  scaled\magstep1          \skewchar\tensy='60
\font\ninesy      =cmsy7  scaled\magstep1         \skewchar\ninesy='60
\font\sevensy     =cmsy6  scaled\magstep1        \skewchar\sevensy='60
\font\sixsy       =cmsy5  scaled\magstep1          \skewchar\sixsy='60
\let\fivesy=\sixsy        % no cmsy4
%
\font\seventeenex =cmex10 scaled\magstep3
\font\fourteenex  =cmex10 scaled\magstep2
\font\twelveex    =cmex10 scaled\magstep1
\let\tenex=\twelveex
%
\font\seventeensl =cmsl12 scaled\magstep2
\font\fourteensl  =cmsl12 scaled\magstep1
\font\twelvesl    =cmsl10 scaled\magstep1
\font\tensl       =cmsl8  scaled\magstep1
\let\ninesl=\ninerm     % no cmsl7
%
\font\seventeenit =cmti12 scaled\magstep2
\font\fourteenit  =cmti12 scaled\magstep1
\font\twelveit    =cmti10 scaled\magstep1
\font\tenit       =cmti8  scaled\magstep1
\font\nineit      =cmti7  scaled\magstep1
%
\font\fourteentt  =cmtt12 scaled\magstep1
\font\twelvett    =cmtt10 scaled\magstep1
\font\tentt       =cmtt8  scaled\magstep1
%
\font\fourteencp  =cmcsc10 scaled\magstep2
\font\twelvecp    =cmcsc10 scaled\magstep1
\let\tencp=\twelvecp      % no cmcsc8
%
\font\tenmsa=msam8 scaled\magstep1
\font\sevenmsa=msam6 scaled\magstep1
\font\fivemsa=msam5 scaled\magstep1
\font\tenmsb=msbm8 scaled\magstep1
\font\sevenmsb=msbm6 scaled\magstep1
\font\fivemsb=msbm5 scaled\magstep1
\font\teneufm=eufm8 scaled\magstep1
\font\seveneufm=eufm6 scaled\magstep1
\font\fiveeufm=eufm5 scaled\magstep1
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\fourteenf@nts{\relax
    \textfont0=\fourteenrm          \scriptfont0=\tenrm
      \scriptscriptfont0=\sevenrm
    \textfont1=\fourteeni           \scriptfont1=\teni
      \scriptscriptfont1=\seveni
    \textfont2=\fourteensy          \scriptfont2=\tensy
      \scriptscriptfont2=\sevensy
    \textfont3=\fourteenex          \scriptfont3=\twelveex
      \scriptscriptfont3=\tenex
    \textfont\itfam=\fourteenit     \scriptfont\itfam=\tenit
    \textfont\slfam=\fourteensl     \scriptfont\slfam=\tensl
    \textfont\bffam=\fourteenbf     \scriptfont\bffam=\tenbf
      \scriptscriptfont\bffam=\sevenbf
    \textfont\ttfam=\fourteentt
    \textfont\cpfam=\fourteencp }
%
\def\twelvef@nts{\relax
    \textfont0=\twelverm          \scriptfont0=\ninerm
      \scriptscriptfont0=\sixrm
    \textfont1=\twelvei           \scriptfont1=\ninei
      \scriptscriptfont1=\sixi
    \textfont2=\twelvesy          \scriptfont2=\ninesy
      \scriptscriptfont2=\sixsy
    \textfont3=\twelveex          \scriptfont3=\tenex
      \scriptscriptfont3=\tenex
    \textfont\itfam=\twelveit     \scriptfont\itfam=\nineit
    \textfont\slfam=\twelvesl     \scriptfont\slfam=\ninesl
    \textfont\bffam=\twelvebf     \scriptfont\bffam=\ninebf
      \scriptscriptfont\bffam=\sixbf
    \textfont\ttfam=\twelvett
    \textfont\cpfam=\twelvecp }
%
\def\tenf@nts{\relax
    \textfont0=\tenrm          \scriptfont0=\sevenrm
      \scriptscriptfont0=\fiverm
    \textfont1=\teni           \scriptfont1=\seveni
      \scriptscriptfont1=\fivei
    \textfont2=\tensy          \scriptfont2=\sevensy
      \scriptscriptfont2=\fivesy
    \textfont3=\tenex          \scriptfont3=\tenex
      \scriptscriptfont3=\tenex
    \textfont\itfam=\tenit     \scriptfont\itfam=\seveni  % no \sevenit
    \textfont\slfam=\tensl     \scriptfont\slfam=\sevenrm % no \sevensl
    \textfont\bffam=\tenbf     \scriptfont\bffam=\sevenbf
      \scriptscriptfont\bffam=\fivebf
    \textfont\ttfam=\tentt
    \textfont\cpfam=\tencp }


==> phyzzx.local.tex <==
%
%  This is the PHYZZX.LOCAL file.
%  It contains local, ie. site-dependent macros.
%
%  This version of the file is for use at SLAC only.
%  Do not use it as is at other sites -- it is distributed only
%  to provide an example of macros you may want to use at your site.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\slacpub{\afterassignment\slacp@b\toks@}
\def\slacp@b{\edef\n@xt{\Pubnum={SLAC--PUB--\the\toks@}}\n@xt}
\let\pubnum=\slacpub
%
\expandafter\ifx\csname eightrm\endcsname\relax
    \let\eightrm=\ninerm \let\eightbf=\ninebf \fi
%
\def\memohead{\hrule height\z@ \kern -0.5in
    \line{\quad\fourteenrm SLAC MEMORANDUM\hfil \twelverm\the\date\quad}}
\def\memorule{\par \medskip \hrule height 0.5pt \kern 1.5pt
   \hrule height 0.5pt \medskip}
%
\def\SLACHEAD{\setbox0=\vtop{\baselineskip=10pt
     \ialign{\eightrm ##\hfil\cr
        \slacbin\cr
        P.^O.^Box 4349\cr
        Stanford, CA 94309\cropen{1\jot}
        \slacphone\cr }}%
   \setbox2=\hbox{\caps Stanford Linear Accelerator Center}%
   \hrule height \z@ \kern -0.5in
   \vbox to 0pt{\vss\centerline{\seventeenrm STANFORD UNIVERSITY}}
   \vbox{} \medskip
   \line{\hbox to 0.7\hsize{\hss \lower 10pt \box2 \hfill }\hfil
         \hbox to 0.25\hsize{\box0 \hfil }}\medskip }
\let\letterhead=\SLACHEAD
%
\FromAddress={\crcr \slacbin \cr
    P.\ O.\ Box 4349\cr Stanford, California 94309\cr }
%
\def\slacbin{SLAC\expandafter\ifx\csname binno\endcsname\relax
                             \else , Bin \binno \fi }
\def\slacphone{(415) 926--\slacext}
\def\slacext{3300}
%
\def\doeack{\foot{Work supported by the Department of Energy,
      contract DE--AC03--76SF00515.}}
%
\VOFFSET=33pt
\papersize
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Now comes the graphic package.
%  This version is rather primitive
%
\newwrite\figscalewrite
\newif\iffigscaleopen
\newif\ifgrayscale
\newif\ifreadyfile
\def\picturedefault{\grayscalefalse \readyfilefalse
    \gdef\ready{\readyfiletrue}\gdef\gray{\ready\grayscaletrue}}
%
\def\parsefilename{\ifreadyfile \else
    \iffigscaleopen \else \gl@bal\figscaleopentrue
       \immediate\openout\figscalewrite=\jobname.scalecon \fi
    \toks0={ }\immediate\write\figscalewrite{%
       \the\p@cwd \the\toks0 \the\p@cht \the\toks0 \the\picfilename }%
    \expandafter\p@rse \the\picfilename..\endp@rse \fi }
%
\def\p@rse#1.#2.#3\endp@rse{%
   \if*#3*\dop@rse #1.1..\else \if.#3\dop@rse #1.1..\else
                                \dop@rse #1.#3\fi \fi
   \expandafter\picfilename\expandafter{\n@xt}}
\def\dop@rse#1.#2..{\count255=#2 \ifnum\count255<1 \count255=1 \fi
   \ifnum\count255<10  \edef\n@xt{#1.PICT00\the\count255}\else
   \ifnum\count255<100 \edef\n@xt{#1.PICT0\the\count255}\else
                       \edef\n@xt{#1.PICT\the\count255}\fi\fi }
%
\def\redopicturebox{\edef\picturedefinition{\ifgrayscale
     \special{insert(\the\picfilename)}\else
     \special{mergeug(\the\picfilename)}\fi }}
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Few miscellaneous macros
%
\let\us=\undertext
\let\rule=\memorule
\let\eqnalign=\eqname
%
\def\pri{^{\, \prime }}
\def\prii{^{\, \prime\, \prime }}
\def\priii{^{\, \prime\, \prime\, \prime }}
\def\epem{{e^+e^-}}
%%
\def\larrow{\leftarrow}
\def\rarrow{\rightarrow }
\def\uarrow{\uparrow }
\def\darrow{\downarrow }
\def\dblarrow{\doublearrow }
\def\longvec{\overrightarrow }
\def\wtilde{\widetilde }
%%
\def\xplus{\becomes{x\rarrow{+\infty}}}
\def\xminus{\becomes{x\rarrow{-\infty}}}
\def\xxx{\becomes{x\rarrow\infty}}
%%
\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern3pt
\vbox{\kern3pt#1\kern3pt}\kern3pt\vrule}\hrule}}
%%

